Calibrating Long Period Variables as Standard Candles with Machine Learning

Variable stars with well-calibrated period-luminosity relationships provide accurate distance measurements to nearby galaxies and are therefore a vital tool for cosmology and astrophysics. While these measurements typically rely on samples of Cepheid and RR-Lyrae stars, abundant populations of luminous variable stars with longer periods of $10 - 1000$ days remain largely unused. We apply machine learning to derive a mapping between lightcurve features of these variable stars and their magnitude to extend the traditional period-luminosity (PL) relation commonly used for Cepheid samples. Using photometric data for long period variable stars in the Large Magellanic cloud (LMC), we demonstrate that our predictions produce residual errors comparable to those obtained on the corresponding Cepheid population. We show that our model generalizes well to other samples by performing a blind test on photometric data from the Small Magellanic Cloud (SMC). Our predictions on the SMC again show small residual errors and biases, comparable to results that employ PL relations fitted on Cepheid samples. The residual biases are complementary between the long period variable and Cepheid fits, which provides exciting prospects to better control sources of systematic error in cosmological distance measurements. We finally show that the proposed methodology can be used to optimize samples of variable stars as standard candles independent of any prior variable star classification.

==> MMRAUVARSTARS 2/trash.tex <==
However this is not equivalent to imposing a transformation of the form Wes -> a Wes ( a < 1), which would indeed change the RMSE alone (Eq. 8). A counter example is the fact that it would change the ME (Eq. 9) in the same manner and the ME is demonstrably very flat as a function of the sample size as can be seen in the right panel of Fig. 4. 


To make this point clearer one can assume a very simple linear regression model like the log(P)-L relation for Cepheids. An arbitrary cut on e.g. log(P) < 1 would not itself decrease the RMSE or the ME, since the intrinsic scatter can very well be independent of the period. 


If such a decrease is detected it can be due to e.g. a different noise level or since the selected sample has some intrinsic property that decreases the width of the conditional distribution. For our selection the noise will not be the reason as the selection of OSARGS lies at fainter magnitudes and has on average quite small amplitudes, which will increase the uncertainty in the feature set (see the discussion in paragraph 5 of the conclusions). Thus the better performance in terms of the RMSE is (very likely) a property of the selected population.


The fact that the fainter end of the OSARG sample shows better correlations between their lightcurve feature and their wesenheit is thus not a limitation of the methodology, but a property of the sample.


==> trash.tex <==
However this is not equivalent to imposing a transformation of the form Wes -> a Wes ( a < 1), which would indeed change the RMSE alone (Eq. 8). A counter example is the fact that it would change the ME (Eq. 9) in the same manner and the ME is demonstrably very flat as a function of the sample size as can be seen in the right panel of Fig. 4. 


To make this point clearer one can assume a very simple linear regression model like the log(P)-L relation for Cepheids. An arbitrary cut on e.g. log(P) < 1 would not itself decrease the RMSE or the ME, since the intrinsic scatter can very well be independent of the period. 


If such a decrease is detected it can be due to e.g. a different noise level or since the selected sample has some intrinsic property that decreases the width of the conditional distribution. For our selection the noise will not be the reason as the selection of OSARGS lies at fainter magnitudes and has on average quite small amplitudes, which will increase the uncertainty in the feature set (see the discussion in paragraph 5 of the conclusions). Thus the better performance in terms of the RMSE is (very likely) a property of the selected population.


The fact that the fainter end of the OSARG sample shows better correlations between their lightcurve feature and their wesenheit is thus not a limitation of the methodology, but a property of the sample.

